Certainty-Equivalence Model Predictive Control: Stability, Performance, and Beyond

Handling model mismatch is a common challenge in model predictive control (MPC). While robust MPC is effective, its conservatism often makes it less desirable. Certainty-equivalence MPC (CE-MPC), which uses a nominal model, offers an appealing alternative due to its design simplicity and low computational costs. This paper investigates CE-MPC for uncertain nonlinear systems with multiplicative parametric uncertainty and input constraints that are inactive at the steady state. The primary contributions are two-fold. First, a novel perturbation analysis of the MPC value function is provided, without assuming the Lipschitz continuity of the stage cost, better tailoring the widely used quadratic cost and having broader applicability in value function approximation, learning-based MPC, and performance-driven MPC design. Second, the stability and performance analysis of CE-MPC are provided, quantifying the suboptimality of CE-MPC compared to the infinite-horizon optimal controller with perfect model knowledge. The results provide insights in how the prediction horizon and model mismatch jointly affect stability and the worst-case performance. Furthermore, the general results are specialized to linear quadratic control, and a competitive ratio bound is derived, serving as the first competitive-ratio bound for MPC of uncertain linear systems with input constraints and multiplicative uncertainty.

==> 1-major_content/8-acknowledgement.tex <==
\section*{Acknowledgment}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/a1.png}}]{First A. Author} (Fellow, IEEE) and all authors may include 
	biographies. Biographies are
	often not included in conference-related papers.
	This author is an IEEE Fellow. The first paragraph
	may contain a place and/or date of birth (list
	place, then date). Next, the author’s educational
	background is listed. The degrees should be listed
	with type of degree in what field, which institution,
	city, state, and country, and year the degree was
	earned. The author’s major field of study should
	be lower-cased.
	
	The second paragraph uses the pronoun of the person (he or she) and
	not the author’s last name. It lists military and work experience, including
	summer and fellowship jobs. Job titles are capitalized. The current job must
	have a location; previous positions may be listed without one. Information
	concerning previous publications may be included. Try not to list more than
	three books or published articles. The format for listing publishers of a book
	within the biography is: title of book (publisher name, year) similar to a
	reference. Current and previous research interests end the paragraph.
	
	The third paragraph begins with the author’s title and last name (e.g.,
	Dr. Smith, Prof. Jones, Mr. Kajor, Ms. Hunter). List any memberships in
	professional societies other than the IEEE. Finally, list any awards and work
	for IEEE committees and publications. If a photograph is provided, it should
	be of good quality, and professional-looking.
\end{IEEEbiography}

\begin{IEEEbiographynophoto}{Second B. Author,} photograph and biography not available at the
	time of publication.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Third C. Author Jr.} (Member, IEEE), photograph and biography not available at the
	time of publication.
\end{IEEEbiographynophoto}

==> 5-appendices/Lemma4_complex.tex <==
\begin{proof}
	The proof employs induction. For $k = 0$, $\xi^{\star}_k(x';\para) = x'$, $\xi^{\star}_k(x'';\para) = x''$, and $\Gamma_{k} = 1$. Thus, \eqref{eq:lm4_open_loop_state_perturbation_bound} holds as an equality for $k = 0$. Assume that \eqref{eq:lm4_open_loop_state_perturbation_bound} holds for $k = k_0$ with $k_0 \in \bI_{0:N-1}$, i.e.,
	\begin{multline}
		\label{eq:B2_induction_assumption}
		\|\xi^\star_{k_0}(x';\para) - \xi^\star_{k_0}(x'';\para)\| \leq \\
		\left((\blfx)^{k_0} + \blfu\edsc\sum^{k_0-1}_{i=0}(\blfx)^i\edsr^{k_0-i}\right)\|x' - x''\|.
	\end{multline}
	Then, for $k = k_0 + 1$, it follows that
	\begin{align}
		& \|\xi^\star_{k_0+1}(x';\para) - \xi^\star_{k_0+1}(x'';\para)\| \notag \\
		= &\; \|f(\xi^\star_{k_0}(x';\para),u^\star_{k_0}(x';\para);\para) \sminus f(\xi^\star_{k_0}(x'';\para),u^\star_{k_0}(x'';\para);\para)\| \notag \\
		& \hspace*{-2.5ex} \overset{\eqref{eq:lipschitz_dynamics}}{\leq} \blfx\|\xi^\star_{k_0}(x';\para) - \xi^\star_{k_0}(x'';\para)\| + \notag \\
		& \hspace*{20ex} \blfu\|u^\star_{k_0}(x';\para) - u^\star_{k_0}(x'';\para)\| \notag \\
		& \hspace*{-1.5ex} \overset{\eqref{eq:subsec_eds:state_sensitivity_input},\eqref{eq:B2_induction_assumption}}{\leq} \left((\blfx)^{k_0+1} + \blfu\edsc\sum^{k_0-1}_{i=0}(\blfx)^{i+1}\edsr^{k_0-i} + \right. \notag \\
		& \hspace*{32ex} \blfu\edsc\edsr^{k_0}\Bigg)\|x' - x''\| \notag \\
		= & \left((\blfx)^{k_0+1} + \blfu\edsc\sum^{k_0}_{i=0}(\blfx)^{i}\edsr^{k_0+1-i} \right)\|x' - x''\|, \notag 
	\end{align}
	which completes the induction relation. A slight modified version of \eqref{eq:lm4_open_loop_state_perturbation_bound} that will be used later is
	\begin{equation}
		\label{eq:B2_final_conclusion}
		\|\xi^\star_{k}(\xp{\hpara};\hpara) - \xi^\star_{k}(\xp{\para};\hpara)\| \leq \Gamma_{k}\|\xp{\hpara} - \xp{\para}\|.
	\end{equation}
\end{proof}

==> 5-appendices/Lemma6_complex.tex <==
\begin{proof}
	For notational convenience, we define
	\begin{subequations}
		\label{eq:C2_definition}
		\begin{align}
			\label{eq:C2_def_state_dif}
			& \hspace*{-2ex} \Delta \xi^\star_{k}(x) := \xi^\star_{k}(x;\para) - \xi^\star_{k}(x;\hpara), \;\forall k \in \bI_{0:N}, \\
			\label{eq:C2_def_input_dif}
			& \hspace*{-2ex} \Delta u^\star_{k}(x) :=  u^\star_{k}(x;\para) - u^\star_{k}(x;\hpara) ,\;\forall k \in \bI_{0:N-1}, \\
			\label{eq:C2_def_pair}
			& \hspace*{-2ex} \Delta^\star_{f,k}(x;\hpara) := \Delta_f(\xi^\star_{k}(x;\hpara), u^\star_{k}(x;\hpara); \para),\;\forall k \in \bI_{0:N-1}.
		\end{align}
	\end{subequations}
	First, we establish the recursive relation between $\difxi{k+1}$ and $\difxi{k}$ as follows.
	\begin{align}
		\label{eq:C2_recursive_relation}
		& \;\difxi{k+1} \notag \\ 
		= & \;\|f(\xi^{\star}_k(x;\para), u^{\star}_k(x;\para); \para) \sminus f(\xi^{\star}_k(x;\hpara), u^{\star}_k(x;\hpara); \hpara)\| \notag \\
		\leq &\; \|f(\xi^{\star}_k(x;\para), u^{\star}_k(x;\para); \para) \sminus f(\xi^{\star}_k(x;\hpara), u^{\star}_k(x;\hpara); \para)\| + \notag \\
		&\; \hspace*{35ex} \dpairf{k} \notag \\
		& \hspace*{-2ex} \overset{\eqref{eq:lipschitz_dynamics}}{\leq}  \; L_{f,x}\difxi{k} + L_{f,u}\difu{k} + \dpairf{k},
	\end{align}
	where the second inequality is due to triangle inequality. Next, the main result \eqref{eq:open_loop_parameter_perturbation_bound} is proven by induction. For $k=0$, $C_{\Delta u,0}(\mpara;x) = 0$, $\sum^{-1}_{i=0}[\cdot] = 0$, and $\xi^\star_{0}(x;\para) - \xi^\star_{0}(x;\hpara) = x - x = 0$. Thus, \eqref{eq:open_loop_parameter_perturbation_bound} holds trivially with both sides equal to $0$. Assume that \eqref{eq:open_loop_parameter_perturbation_bound} holds for $k = k_0$, i.e.,
	\begin{multline}
		\label{eq:C2_induction_assumption}
		\difxi{k_0} \leq L_{f,u}\sum^{k_0-1}_{i=0}L^{k_0-1-i}_{f,x}\sueds{i}(\mpara;\|x\|) + \\ \sum^{k_0-1}_{i=0}L^{k_0-1-i}_{f,x}\|\Delta f(\xi^\star_{i}(x;\hpara),u^\star_{i}(x;\hpara);\para)\|.
	\end{multline}
	Then, for $k = k_0 + 1$, it holds that
	\begin{align}
		% \label{eq:C2_induction_prove}
		& \hspace*{4ex} \difxi{k_0+1} \notag \\
		& \overset{\eqref{eq:C2_recursive_relation}}{\leq} L_{f,x}\difxi{k_0} + L_{f,u}\difu{k_0} + \dpairf{k_0} \notag \\
		&  \overset{\eqref{eq:C2_induction_assumption}}{\leq} L_{f,u}\sum^{k_0-1}_{i=0}L^{k_0-i}_{f,x}\sueds{i}(\mpara;\|x\|) \splus \sum^{k_0-1}_{i=0}L^{k_0-i}_{f,x}\dpairf{i} \notag \\
		& \hspace*{5ex} + L_{f,u}\difu{k_0} + \dpairf{k_0} \notag \\ 
		&  \overset{\eqref{eq:subsec_para_perturbation:refined_eds}}{\leq} L_{f,u}\sum^{k_0-1}_{i=0}L^{k_0-i}_{f,x}\sueds{i}(\mpara;\|x\|) \splus \sum^{k_0-1}_{i=0}L^{k_0-i}_{f,x}\dpairf{i} \notag \\
		& \hspace*{5ex} + L_{f,u}\sueds{k_0}(\mpara; \|x\|) + \dpairf{k_0} \notag \\
		& \hspace*{1ex} \leq L_{f,u}\sum^{k_0}_{i=0}L^{k_0-i}_{f,x}\sueds{i}(\mpara;\|x\|) + \sum^{k_0}_{i=0}L^{k_0-i}_{f,x}\dpairf{i}, \notag
	\end{align}
	which completes the induction relation.
\end{proof}

==> 5-appendices/Prop2_complex.tex <==
\begin{proof}
	The left inequality of \eqref{eq:nominal_bound} is due to
	\begin{equation*}
		\cost^\star(x) \leq \cost(x, \mu_{N,\hpara}(x)) \leq V_{N}(x;\para),
	\end{equation*}
	and the right inequality is a direct consequence of \eqref{eq:sec_prob:mpc_linear_bound}. To prove \eqref{eq:nominal_decreasing}, we employ the \textit{case distinction} method in \cite{kohler2023stability}. More specifically, the final cost evaluated at stage $N$, i.e., $\cost^\star(\xi^\star_N(x;\hpara))$, is used as the distinction variable. First, assume that
	\begin{equation}
		\label{eq:B1_case1_assumption}
		\cost^\star(\xi^\star_N(x;\hpara)) \leq \frac{(1 + \umpc)\mpc_{N}}{(N -1)\lyacf + N + \umpc}\cost^\star(x).
	\end{equation}
	By definition, it holds that
	\begin{multline}
		\label{eq:B1_firstcase_ground}
		V_N(\xp{\hpara};\hpara) =  \cost^\star(\xi^\star_N(\xp{\hpara};\hpara)) + \\ \sum^{N-1}_{k=0}\cost(\xi^\star_k(\xp{\hpara};\hpara), u^\star_k(\xp{\hpara};\hpara)).
	\end{multline}
	Due to the optimality of $\mathbf{u}^\star_N(\xp{\hpara};\hpara)$, \eqref{eq:B1_firstcase_ground} implies that
	\begin{align}
		\label{eq:B1_firstcase_main_derivation}
		& V_N(\xp{\hpara};\hpara) \notag \\
		\leq & \; \cost^\star(f(\xi^\star_N(x;\hpara), \uclf;\hpara) + \notag \\
		& \;\cost(\xi^\star_N(x;\hpara), \uclf) + \sum^{N-1}_{k=1}\cost(\xi^\star_{k}(x;\hpara), u^\star_{k}(x;\hpara)) \notag \\
		\leq &  \; \cost^\star(f(\xi^\star_N(x;\hpara), \uclf;\hpara) + \cost(\xi^\star_N(x;\hpara), \uclf) + \notag \\
		& \;V_N(x;\hpara) - \cost(x, \mu_{N,\hpara}(x)) - \cost^\star(\xi^\star_N(x;\hpara)) \notag \\
		\overset{\eqref{eq:sec_prob:relaxed_clf}}{\leq} & \;\lyacf \cost^\star(\xi^\star_N(x;\hpara)) + V_N(x;\hpara) - \cost(x, \mu_{N,\hpara}(x)),
	\end{align}
	where the second inequality is due to the definition of $V_N(x;\hpara)$. \eqref{eq:B1_firstcase_main_derivation} is equivalent to
	\begin{align}
		\label{eq:B1_firstcase_final}
		& \;V_N(\xp{\hpara};\hpara) - V_N(x;\hpara) \notag \\ 
		\leq  & \; - \cost(x, \mu_{N,\hpara}(x)) + \lyacf \cost^\star(\xi^\star_N(x;\hpara)) \notag \\
		\overset{\eqref{eq:B1_case1_assumption}}{\leq} & \; - \cost(x, \mu_{N,\hpara}(x)) + \frac{(1 + \umpc)\mpc_{N}\lyacf}{(N -1)\lyacf + N + \umpc}\cost^\star(x) \notag \\
		\leq &\; -(1 - \epsilon_N)\cost(x, \mu_{N,\hpara}(x)),
	\end{align}
	where $\epsilon_N := \frac{(1 + \umpc)\mpc_{N}\lyacf}{(N -1)\lyacf + N + \umpc}$. On the other hand, assume that
	\begin{equation}
		\label{eq:B1_case2_assumption}
		\cost^\star(\xi^\star_N(x;\hpara)) \geq \frac{(1 + \umpc)\mpc_{N}}{(N -1)\lyacf + N + \umpc}\cost^\star(x).
	\end{equation}
	By definition, it holds that
	\begin{multline}
		\label{eq:B1_case2_ground}
		\sum^{N-1}_{k=0}\cost^\star(\xi^\star_k(x;\hpara)) \leq V_N(x;\hpara) - \cost^\star(\xi^\star_N(x;\hpara)) \\
		\overset{\eqref{eq:sec_prob:mpc_linear_bound},\eqref{eq:B1_case2_assumption}}{\leq} \left(1 + \mpc_{N} - \frac{(1 + \umpc)\mpc_{N}}{(N -1)\lyacf + N + \umpc}\right)\cost^\star(x).
	\end{multline}
	Subtracting $\cost^\star(x)$ on both sides of \eqref{eq:B1_case2_ground} yields
	\begin{equation}
		\label{eq:B1_case2_turnpoint}
		\sum^{N-1}_{k=1}\cost^\star(\xi^\star_k(x;\hpara)) \leq \frac{\mpc_{N}(1 + \lyacf)(N -1)}{(N-1)\lyacf + N + \umpc}\cost^\star(x),
	\end{equation} 
	which indicates that $\exists k^\ast \in \bI_{1:N-1}$ such that
	\begin{equation}
		\label{eq:B1_case2_turnpoint_base}
		\cost^\star(\xi^\star_{k^\ast}(x;\hpara)) \leq \frac{\mpc_{N}(1 + \lyacf)}{(N-1)\lyacf + N + \umpc}\cost^\star(x).
	\end{equation}
	Then, it holds that
	\begin{align}
		& \;V_{N}(\xp{\hpara}) + \cost(x, \mu_{N,\hpara}(x)) \notag \\
		\leq &\; J_{k^\ast}(x, \mathbf{u}^\ast_N(x;\hpara)) + V_{N-k^\ast+1}(\cost^\star(\xi^\star_{k^\ast}(x;\hpara))) \notag \\
		\overset{\eqref{eq:sec_prob:mpc_linear_bound}}{\leq} &\; V_N(x;\hpara) - \cost^\star(\xi^\star_N(x;\hpara)) + (1 + \umpc) \cost^\star(\xi^\star_{k^\ast}(x;\hpara)) \notag \\
		&\hspace*{-2ex} \overset{\eqref{eq:B1_case2_assumption},\eqref{eq:B1_case2_turnpoint_base}}{\leq} \; V_N(x;\hpara) + \frac{(1 + \umpc)\mpc_{N}\lyacf}{(N -1)\lyacf + N + \umpc}\cost^\star(x),
	\end{align}
	which again implies that
	\begin{equation}
		\label{eq:B1_case2_conclusion}
		V_N(\xp{\hpara};\hpara) - V_N(x;\hpara) \leq -(1 - \epsilon_N)\cost(x, \mu_{N,\hpara}(x)).
	\end{equation}
	Therefore, in both cases the desired property \eqref{eq:B1_case2_conclusion} (cf. \eqref{eq:nominal_decreasing}) is established. Besides, it holds that
	\begin{align}
		\label{eq:B3_energy_decreasing}
		& \;V_N(\xp{\hpara};\hpara) \notag \\
		\overset{\eqref{eq:B1_case2_conclusion}}{\leq} & \;V_N(x;\hpara) - (1 - \epsilon_N)\cost(x, \mu_{N,\hpara}(x))\notag  \\ 
		\overset{\eqref{eq:sec_prob:mpc_linear_bound}}{\leq} & \;(1 + \mpc_N)\cost^\star(x) - (1 - \epsilon_N)\cost(x, \mu_{N,\hpara}(x))\notag  \\ 
		\leq & \;(1 + \mpc_N)\cost(x, \mu_{N,\hpara}(x)) - (1 - \epsilon_N)\cost(x, \mu_{N,\hpara}(x))\notag  \\ 
		\leq & \;(\mpc_N + \epsilon_N)\cost(x, \mu_{N,\hpara}(x)),
	\end{align}
	which completes the proof.
\end{proof}

==> unused.tex <==
% unused text
One sufficient condition to ensure Assumption \ref{ass:sec_prob:nominal_cost_controllability} is the exponential decay of stage cost \cite{grune2012nmpc, kohler2021stability}, specifically, if there exist constants $C \geq 1$ and $\sigma \in (0,1)$ such that for all $x \in \xroa$ and each $N \in \bN$ there is an input sequence $\bu \in \cU^N$ such that 
\begin{equation}
	\label{eq:sec_prob:exponential_decay_stage_cost}
	l(\otx{\hpara}(k;x,\bu[0:k-1]),\bu[k]) \leq C \sigma^{k}l^\ast(x)
\end{equation}
holds for $k \in \bI_{0:N-1}$. Under this condition, Assumption \ref{ass:sec_prob:nominal_cost_controllability} is valid with $\mpc_i = \frac{C+\sigma-\sigma^i}{1 - \sigma}$. A generalized version of \eqref{eq:sec_prob:exponential_decay_stage_cost} and more detailed discussions are provided in Appendix \qt{[?]}.

The set of positive definite functions $\pdf{d}$ is defined as $\pdf{d} = \{\alpha: \bR^d \to \bR_+ \mid \alpha(x) = 0 \iff x = \mathbf{0}\}$.

\footnote{Denote the minimizer of the left-hand-side of Eq. \eqref{eq:sec_prob:relaxed_clf} as $\uclf$, and Eq. \eqref{eq:sec_prob:relaxed_clf} can be written as $\ell^\star(x^+(\uclf;\hpara)) - \ell^\star(x) \leq -l(x, \uclf) + \lyacf \ell^\star(x)$, where $\uclf$ implicitly defines a terminal control policy.}

%% Proofs
\subsection{Proof of Lemma \ref{lm:lipschitz_gradient}}
\label{appendix:A1}
\begin{proof}
	Following \cite[Lemma 1.2.3]{nesterov2013introductory}, if $\cost \in C^{1,1}_{L}(\bR^n \times \bR^m)$ and $\Vf \in C^{1,1}_{L}(\bR^n)$, it holds that
	\begin{subequations}
		\label{eq:A1_cost_specification}
		\begin{multline}
			\label{eq:A1_cost_specification_stage_cost}
			|\cost(x + \delta_x, u + \delta_u) - \cost(x, u) - [\nabla_x^\top \cost, \nabla_u^\top \cost][\delta x^\top,\delta u^\top]^\top| \leq \\ \frac{L_{\nabla\ell}}{2}\|[\delta_x^\top, \delta_u^\top]^\top\|^2,
		\end{multline}
		\begin{equation}
			\label{eq:A1_cost_specification_terminal_cost}
			|\Vf(x + \delta_x) - \Vf(x) - \nabla_x^\top\Vf \cdot \delta_x| \leq \frac{L_{\nabla\Vf}}{2}\|x\|^2,
		\end{equation}
	\end{subequations}
	where $L_{\nabla\ell}$ and $L_{\nabla\Vf}$ are, respectively, the Lipschitz constant of $\nabla \cost$ and $\nabla\Vf$. From \eqref{eq:A1_cost_specification_stage_cost} and \eqref{eq:A1_cost_specification_terminal_cost}, by Cauchy-Schwarz inequality and triangle inequality it can be obtained that
	\begin{subequations}
		\label{eq:A1_cost_specification_rewrite}
		\begin{multline}
			\label{eq:A1_cost_specification_stage_cost_rewrite}
			|\cost(x + \delta_x, u + \delta_u) - \cost(x, u)| \leq L_{\nabla\ell}\left(\|\delta_x\|^2 + \|\delta_u\|^2\right) + \\ \|[\nabla_x^\top \cost, \nabla_u^\top \cost]\|\left(\|\delta_x\| + \|\delta_u\|\right),
		\end{multline}
		\begin{equation}
			\label{eq:A1_cost_specification_terminal_cost_rewrite}
			|\Vf(x + \delta_x) - \Vf(x)| \leq \frac{L_{\nabla\Vf}}{2}\|x\|^2 + \\ \|\nabla_x \Vf\|\|\delta_x\|.
		\end{equation}
	\end{subequations}
	As such, \eqref{eq:A1_cost_specification_rewrite} directly implies that Assumption \ref{ass:sec_analysis:bounded_perturbed_stage_cost} holds with $\dlb(\|\delta_x\|, \|\delta_u\|) = L_{\nabla\ell}\left(\|\delta_x\|^2 + \|\delta_u\|^2\right)$, $\dls(\|\delta_x\|, \|\delta_u\|) = \|\delta_x\| + \|\delta_u\|$, $\Bl(x, u) = \|[\nabla_x^\top \cost, \nabla_u^\top \cost]\|$, $\dvfb(\|\delta_x\|) = \frac{L_{\nabla\Vf}}{2}\|x\|^2$, $\dvfs(\|\delta_x\|) = \|\delta_x\|$, and $\Bvf(x) = \|\nabla_x \Vf\|$.
\end{proof}

